ROSA Analyser: An automatized approach to analyse processes of ROSA

In this work we present the first version of ROSA Analyser, a tool designed to get closer to a fully automatic process of analysing the behaviour of a system specified as a process of the Markovian Process Algebra ROSA. In this first development stage, ROSA Analyser is able to generate the Labelled Transition System, according to ROSA Operational Semantics. ROSA Analyser performance starts with the Syntactic Analysis so generating a layered structure, suitable to then, apply the Operational Semantics Transition rules in the easier way. ROSA Analyser is able to recognize some states identities deeper than the Syntactic ones. This is the very first step in the way to reduce the size of the LTS and then to avoid the state explosion problem, so making this task more tractable. For the sake of better illustrating the usefulness of ROSA Analyser, a case study is also provided within this work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{C. Andr\'es and L. Llana (Eds.): 2nd Workshop on Formal\\
Methods in the Development of Software 2012 (WS-FMDS 2012).\\
EPTCS 86, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.86.4}{10.4204/EPTCS.86.4}}
\pdfoutput=1

